Characterizing Impacts of Storage Faults on HPC Applications: A Methodology and Insights

In recent years, the increasing complexity in scientific simulations and emerging demands for training heavy artificial intelligence models require massive and fast data accesses, which urges high-performance computing (HPC) platforms to equip with more advanced storage infrastructures such as solid-state disks (SSDs). While SSDs offer high-performance I/O, the reliability challenges faced by the HPC applications under the SSD-related failures remains unclear, in particular for failures resulting in data corruptions. The goal of this paper is to understand the impact of SSD-related faults on the behaviors of complex HPC applications. To this end, we propose FFIS, a FUSE-based fault injection framework that systematically introduces storage faults into the application layer to model the errors originated from SSDs. FFIS is able to plant different I/O related faults into the data returned from underlying file systems, which enables the investigation on the error resilience characteristics of the scientific file format. We demonstrate the use of FFIS with three representative real HPC applications, showing how each application reacts to the data corruptions, and provide insights on the error resilience of the widely adopted HDF5 file format for the HPC applications.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
We quantitatively examine the impact of various SSD-related fault models on applications of QMCPACK, Montage, and Nyx in \S\ref{sec:eval}. 
In this section, we extend the discussion to future large scale system design and the potential benefits that are enabled by this study.

\subsection{Storage Hardware Selection}
Over the past years, we have seen NAND flash memory being deployed in high performance computing (HPC) systems in the form of memory extension or non-volatile storage as burst buffer. 
The evolutionary NAND flash technology dramatically increases the storage capacity while at the cost of lifetime.
The number of bits stored per NAND memory cell increases from the 1-bit single-level cell (SLC), 2-bit in multi-level cell (MLC), 3-bit triple-level cell (TLC), to 4-bit quadruple-level cell (QLC).
In contrast, the lifetime of a NAND flash memory device, which is determined by the program/erase (P/E) cycles, is estimated $\sim100,000$ for SLC, $\sim3,000-10,000$ for MLC, $\sim1,000-3,000$ TLC, and $\sim1,000$ for QLC~\cite{cai2017errors, yoon2012advanced}.
The bit error rate increases as the NAND flash memory wears out and eventually exceeds the capability of ECC, which makes it infeasible to determine if the stored data is 0 or 1 on SLC.
The price also varies between the cell types. E.g., the dollars-per-GB of TLC can be 2x of QLC.
Therefore, it is challenging for a data center (e.g., a supercomputing center) or on-premise computing facility with dedicated applications (e.g., LSST telescope or Genome Sequencing Lab) to make optimal storage hardware procurement plan.

The results of this study enable the computing system architects to view the overall application failure rate as the product of a conditional probability $P(Failure|Fault)$ and the fault rate $P(Fault)$, which can be inferred from
existing study on NAND flash device failure rate~\cite{cai2012error, grupp2009characterizing, mielke2008bit}.
Thus the system architects can estimate the application failure rate on each type of the NAND flash device numerically and determine the acceptable failure rate given the actual applications. With the application-specific error resilience characteristics provided by this study, the HPC system designers and application developers can identify a new trade-off point: the applications that are more resilient to SSD-related failures, (i.e. the application experiences low probability of SDCs) may afford to run on the devices featuring larger number of bits in a storage cell, to take advantage of the spatial benefits.  
%~\zhao{Here, we can give a example with Montage assuming LSST is running it. But I can't find a reasonable bit flip rate of MLC or TLC online. The Intel and Micron white papers don't give numbers. A paper says MLC has $10^{-15}$ uncorrectable error rate, but we want the error rate by the end of SSD lifetime, I think.}



\subsection{Implication on ECC-related overhead}

Similar to DRAM, Modern SSDs exploit ECC schemes to mitigate the impact of hardware faults. While effective, one of the downside with the ECC schemes is the associated overhead incurred. For example, the area overhead for parity bits in an 8 KB page can be up to 12\%~\cite{ssd-area}; in terms of the performance overhead for ECC decoding, it contributes to 38\% of the overall access time~\cite{ssd-perf} per every read operation; as of energy consumption, Mathur et. al.~\cite{ssd-energy} shows that the NAND flash memory with ECC can consume seven times more energy in read access, and four times more energy in write access, compared with ones without ECC. 

With the insights gained from our study, it is possible for the SSD designers to explore the opportunity to take a adjustable view on the ECC scheme and enable a software-hardware co-design on SSDs: for applications that have low likelihood of SDC outcomes when affected by SSD-related failures, the frequency of applying ECC schemes on the storage data can be reduced (i.e. not per every read) to mitigate the overall energy consumption; while for other applications that are more likely to detect the errors, it might be also beneficial to tune down the ECC frequency and allow the application level checks to guard the correctness of the application.  


